Valuation Duration of the Stock Market

At the peak of the tech bubble, only 0.57% of market valuation comes from dividends in the next year. Taking the ratio of total market value to the value of one-year dividends, we obtain a valuation-based duration of 175 years. In contrast, at the height of the global financial crisis, more than 2.2% of market value is from dividends in the next year, implying a duration of 46 years. What drives valuation duration? We find that market participants have limited information about cash flow beyond one year. Therefore, an increase in valuation duration is due to a decrease in the discount rate rather than good news about long-term growth. Accordingly, valuation duration negatively predicts annual market return with an out-of-sample R2 of 15%, robustly outperforming other predictors in the literature. While the price-dividend ratio reflects the overall valuation level, our valuation-based measure of duration captures the slope of the valuation term structure. We show that valuation duration, as a discount rate proxy, is a critical state variable that augments the price-dividend ratio in spanning the (latent) state space for stock-market dynamics.

==> Tables/tab_pred_dg12.tex <==
\begin{tabular}{p{4cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
	\toprule
	                                         & \multicolumn{5}{c}{$\log(D_{t+1}/D_t)$}                                                      \\\cmidrule{2-7}
	{}                                       & (1)                                     & (2)     & (3)      & (4)     & (5)      & (6)      \\ \midrule
	% Intercept                                 & 0.208    & 0.010    & 0.050    & 0.137   & 0.080    & -0.271    \\
	%                                           & [5.969]  & [-0.513] & [11.347] & [3.637] & [20.549] & [-11.875] \\
	%                                           & (2.906)  & (0.046)  & (3.710)  & (1.456) & (6.744)  & (-1.287)  \\
	$ dr_t$                                  & -0.036                                  &         &          &         &          & 0.092    \\
	\quad \quad \textit{\small Hodrick t}    & [-4.374]                                &         &          &         &          & [13.702] \\
	\quad \quad \textit{\small Newey-West t} & (-2.091)                                &         &          &         &          & (1.659)  \\
	$pd_t$                                   &                                         & 0.014   &          &         &          &          \\
	                                         &                                         & [1.525] &          &         &          &          \\
	                                         &                                         & (0.250) &          &         &          &          \\
	$g^{F}_{t}$                              &                                         &         & 0.666    &         &          &          \\
	                                         &                                         &         & [14.478] &         &          &          \\
	                                         &                                         &         & (2.850)  &         &          &          \\
	$KP_t$                                   &                                         &         &          & 0.149   &          &          \\
	                                         &                                         &         &          & [1.861] &          &          \\
	                                         &                                         &         &          & (0.839) &          &          \\
	$\ln \left(\frac{D_t}{P^{T-}_t}\right)$  &                                         &         &          &         & 0.126    & 0.265    \\
	                                         &                                         &         &          &         & [12.150] & [19.276] \\
	                                         &                                         &         &          &         & (3.404)  & (2.528)  \\\addlinespace[2ex]
	$N$                                      & 384                                     & 384     & 384      & 384     & 384      & 384      \\
	$R^2$                                    & 0.064                                   & 0.003   & 0.303    & 0.020   & 0.250    & 0.362    \\
	OOS $R^2$                                & 0.050                                   & -0.045  & 0.196    & -0.048  & 0.235    & 0.294    \\
	ENC                                      & 1.597                                   & -0.179  & 3.336    & 1.693   & 5.752    & 7.797    \\
	$p(ENC)$                                 & $<$0.10                                 & $>$0.10 & $<$0.05  & $<$0.10 & $<$0.01  & $<$0.01  \\
	$p(CW)$                                  & 0.065                                   & 0.398   & 0.006    & 0.150   & 0.003    & 0.003    \\
	\bottomrule
\end{tabular}
\label{tb:divg}

==> Tables/tab_pred_dg_mkt12.tex <==
% --> overleaf::tab_pred_dg_mkt12.tex
% \begin{tabular}{lrrrrrr}
\begin{tabular}{p{4cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
    \toprule
                                             & \multicolumn{5}{c}{$\log(D^{MKT}_{t+1}/D^{MKT}_t)$}                                                   \\\cmidrule{2-7}
    {}                                       & (1)                                                 & (2)     & (3)     & (4)     & (5)     & (6)     \\ \midrule
    % Intercept                                & 0.152    & -0.135   & 0.051   & 0.152   & 0.078   & -0.441   \\
    %                                          & [1.635]  & [-1.658] & [4.390] & [1.909] & [7.805] & [-5.655] \\
    %                                          & (1.529)  & (-0.583) & (3.337) & (1.566) & (5.185) & (-2.187) \\
    $ dr_t$                                  & -0.023                                              &         &         &         &         & 0.136   \\
    \quad \quad \textit{\small Hodrick t}    & [-0.939]                                            &         &         &         &         & [6.254] \\
    \quad \quad \textit{\small Newey-West t} & (-0.921)                                            &         &         &         &         & (2.505) \\
    $pd_t$                                   &                                                     & 0.050   &         &         &         &         \\
                                             &                                                     & [2.112] &         &         &         &         \\
                                             &                                                     & (0.836) &         &         &         &         \\
    $g^{F}_{t}$                              &                                                     &         & 0.520   &         &         &         \\
                                             &                                                     &         & [4.513] &         &         &         \\
                                             &                                                     &         & (2.084) &         &         &         \\
    $KP_t$                                   &                                                     &         &         & 0.182   &         &         \\
                                             &                                                     &         &         & [1.127] &         &         \\
                                             &                                                     &         &         & (1.004) &         &         \\
    $\ln \left(\frac{D_t}{P^{T-}_t}\right)$  &                                                     &         &         &         & 0.122   & 0.328   \\
                                             &                                                     &         &         &         & [4.492] & [7.768] \\
                                             &                                                     &         &         &         & (3.419) & (3.401) \\\addlinespace[2ex]
    $N$                                      & 384                                                 & 384     & 384     & 384     & 384     & 384     \\
    $R^2$                                    & 0.017                                               & 0.030   & 0.129   & 0.020   & 0.164   & 0.335   \\
    OOS $R^2$                                & -0.025                                              & -0.027  & 0.027   & -0.063  & 0.126   & 0.273   \\
    ENC                                      & -0.078                                              & -0.278  & 0.727   & 0.508   & 4.035   & 10.014  \\
    $p(ENC)$                                 & >0.10                                               & >0.10   & >0.10   & >0.10   & <0.01   & <0.01   \\
    $p(CW)$                                  & 0.401                                               & 0.213   & 0.099   & 0.315   & 0.004   & 0.003   \\
    \bottomrule
\end{tabular}
\label{tb:divg mkt}

==> Tables/tab_pred_divstrip.tex <==
\begin{tabular}{p{4cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
    \toprule
                                              & \multicolumn{5}{c}{Log Holding Period Return: $\log(D_{t+1}/S^{1}_t)$}                                                  \\\cmidrule{2-6}
    {}                                        & (1)                                                                & (2)     & (3)      & (4)      & (5)            \\
    \midrule
    % 	Intercept &    -1.616 &    -1.756 &    -0.053 &    -0.813 &    -0.306 \\
    % 	&  (-8.396) &  (-3.466) &  (-1.014) &  (-2.433) &  (-1.307) \\
    $ dr_t$                                   & 0.451                                                              &         &          &          & 0.817          \\
    \quad \quad \textit{\small  Newey-West t} & (9.406)                                                            &         &          &          & (15.237)       \\
    $pd_t$                                    &                                                                    & 0.504   &          &          & -0.716         \\
                                              &                                                                    & (3.770) &          &          & (-6.443)       \\
    $\mu^{F}_{t}$                             &                                                                    &         & -6.516   &          &                \\
                                              &                                                                    &         & (-4.230) &          &                \\
    $KP_t$                                    &                                                                    &         &          & -2.031   &                \\
                                              &                                                                    &         &          & (-2.898) &                \\\addlinespace[1ex]
    $N$                                       & 372                                                                & 372     & 372      & 372      & 372       \\
    $R^2$                                     & 0.751                                                              & 0.320   & 0.358    & 0.277    & 0.905          \\
    OOS $R^2$                                 & 0.725                                                              & 0.251   & 0.284    & 0.159    & 0.898          \\
    ENC                                       & 103.462                                                            & 10.821  & 13.089   & 11.984   & 313.972        \\
    $p(ENC)$                                  & $<$0.01                                                            & $<$0.01 & $<$0.01  & $<$0.01  & $<$0.01        \\
    $p(CW)$                                   & 0.023                                                              & 0.030   & 0.030    & 0.031    & 0.031          \\
    \bottomrule
\end{tabular}
